On BTI Aging Rejuvenation in Memory Address Decoders

Memory designs require timing margins to compensate for aging and fabrication process variations. With technology downscaling, aging mechanisms became more apparent, and larger margins are considered necessary. This, in return, means a larger area requirement and lower performance for the memory. Bias Temperature Instability (BTI) is one of the main contributors to aging, which slows down transistors and ultimately causes permanent faults. In this paper, first, we propose a low-cost aging mitigation scheme, which can be applied to existing hardware to mitigate aging on memory address decoder logic. We mitigate the BTI effect on critical transistors by applying a rejuvenation workload to the memory. Such an auxiliary workload is executed periodically to rejuvenate transistors that are located on critical paths of the address decoder. Second, we analyze workloads' efficiency to optimize the mitigation scheme. Experimental results performed with realistic benchmarks demonstrate several-times lifetime extension with a negligible execution overhead.

==> bibliography.tex <==
% First paragraph

@INPROCEEDINGS{SH13,  author={S. {Hamdioui} and D. {Gizopoulos} and G. {Guido} and M. {Nicolaidis} and A. {Grasset} and P. {Bonnot}},  booktitle={2013 Design, Automation   Test in Europe Conference   Exhibition (DATE)},  title={Reliability challenges of real-time systems in forthcoming technology nodes},   year={2013},  volume={},  number={},  pages={129-134},}
% https://ieeexplore.ieee.org/document/6513486

@ARTICLE{KB06,  author={K. {Bernstein} and D. J. {Frank} and A. E. {Gattiker} and W. {Haensch} and B. L. {Ji} and S. R. {Nassif} and E. J. {Nowak} and D. J. {Pearson} and N. J. {Rohrer}},  journal={IBM Journal of Research and Development},  title={High-performance CMOS variability in the 65-nm regime and beyond},   year={2006},  volume={50},  number={4.5},  pages={433-449},}
% https://ieeexplore.ieee.org/document/5388739

@ARTICLE{KKK10,  author={K. K. {Kim} and W. {Wang} and K. {Choi}},  journal={IEEE Transactions on Circuits and Systems II: Express Briefs},  title={On-Chip Aging Sensor Circuits for Reliable Nanometer MOSFET Digital Circuits},   year={2010},  volume={57},  number={10},  pages={798-802},}
% https://ieeexplore.ieee.org/document/5587880


@INPROCEEDINGS{WN98,  author={W. {Needham} and C. {Prunty} and  {Eng Hong Yeoh}},  booktitle={Proceedings International Test Conference 1998 (IEEE Cat. No.98CH36270)},  title={High volume microprocessor test escapes, an analysis of defects our tests are missing},   year={1998},  volume={},  number={},  pages={25-34},}
% https://ieeexplore.ieee.org/document/743133

@INPROCEEDINGS{AJG04,  author={A. J. {van de Goor} and S. {Hamdioui} and R. {Wadsworth}},  booktitle={2004 International Conferce on Test},  title={Detecting faults in the peripheral circuits and an evaluation of SRAM tests},   year={2004},  volume={},  number={},  pages={114-123},}
% https://ieeexplore.ieee.org/document/1386943

% Aging in SRAM

@INPROCEEDINGS{SVK06,  author={S. V. {Kumar} and K. H. {Kim} and S. S. {Sapatnekar}},  booktitle={7th International Symposium on Quality Electronic Design (ISQED'06)},  title={Impact of NBTI on SRAM read stability and design for reliability},   year={2006},  volume={},  number={},  pages={6 pp.-218},}
% https://ieeexplore.ieee.org/document/1613138

@INPROCEEDINGS{IA13,  author={I. {Agbo} and S. {Khan} and S. {Hamdioui}},  booktitle={2013 8th IEEE Design and Test Symposium},  title={BTI impact on SRAM sense amplifier},   year={2013},  volume={},  number={},  pages={1-6},}
% https://ieeexplore.ieee.org/document/6727094

@INPROCEEDINGS{SK13,  author={S. {Khan} and M. {Taouil} and S. {Hamdioui} and H. {Kukner} and P. {Raghavan} and F. {Catthoor}},  booktitle={2013 8th IEEE Design and Test Symposium},  title={Impact of partial resistive defects and Bias Temperature Instability on SRAM decoder reliablity},   year={2013},  volume={},  number={},  pages={1-6},}
% https://ieeexplore.ieee.org/document/6727124

@INPROCEEDINGS{SK14,  author={S. {Khan} and I. {Agbo} and S. {Hamdioui} and H. {Kukner} and B. {Kaczer} and P. {Raghavan} and F. {Catthoor}},  booktitle={2014 Design, Automation   Test in Europe Conference   Exhibition (DATE)},  title={Bias Temperature Instability analysis of FinFET based SRAM cells},   year={2014},  volume={},  number={},  pages={1-6},}
% https://ieeexplore.ieee.org/document/6800245

@INPROCEEDINGS{IA14,  author={I. {Agbo} and M. {Taouil} and S. {Hamdioui} and H. {Kukner} and P. {Weckx} and P. {Raghavan} and F. {Catthoor}},  booktitle={2015 IEEE 33rd VLSI Test Symposium (VTS)},  title={Integral impact of BTI and voltage temperature variation on SRAM sense amplifier},   year={2015},  volume={},  number={},  pages={1-6},}
% https://ieeexplore.ieee.org/document/7116291

@ARTICLE{JD15,  author={J. {Ding} and D. {Reid} and P. {Asenov} and C. {Millar} and A. {Asenov}},  journal={IEEE Transactions on Electron Devices},  title={Influence of Transistors With BTI-Induced Aging on SRAM Write Performance},   year={2015},  volume={62},  number={10},  pages={3133-3138},}
% https://ieeexplore.ieee.org/document/7194785

@ARTICLE{IA17,  author={I. {Agbo} and M. {Taouil} and D. {Kraak} and S. {Hamdioui} and H. {Kükner} and P. {Weckx} and P. {Raghavan} and F. {Catthoor}},  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},  title={Integral Impact of BTI, PVT Variation, and Workload on SRAM Sense Amplifier},   year={2017},  volume={25},  number={4},  pages={1444-1454},}
% https://ieeexplore.ieee.org/document/7819518

@INPROCEEDINGS{JK17,  author={J. {Kinseher} and L. {Heiß} and I. {Polian}},  booktitle={Design, Automation   Test in Europe Conference   Exhibition (DATE), 2017},  title={Analyzing the effects of peripheral circuit aging of embedded SRAM architectures},   year={2017},  volume={},  number={},  pages={852-857},}
% https://ieeexplore.ieee.org/document/7927106

@ARTICLE{DK19,  author={D. {Kraak} and M. {Taouil} and I. {Agbo} and S. {Hamdioui} and P. {Weckx} and S. {Cosemans} and F. {Catthoor}},  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},  title={Parametric and Functional Degradation Analysis of Complete 14-nm FinFET SRAM},   year={2019},  volume={27},  number={6},  pages={1308-1321},}
% https://ieeexplore.ieee.org/document/8678671


% Mitigation for memory cells

@INPROCEEDINGS{AG15,  author={A. {Gebregiorgis} and M. {Ebrahimi} and S. {Kiamehr} and F. {Oboril} and S. {Hamdioui} and M. B. {Tahoori}},  booktitle={The 20th Asia and South Pacific Design Automation Conference},  title={Aging mitigation in memory arrays using self-controlled bit-flipping technique},   year={2015},  volume={},  number={},  pages={231-236},}
% https://ieeexplore.ieee.org/document/7059010

@ARTICLE{AV17,  author={A. {Valero} and N. {Miralaei} and S. {Petit} and J. {Sahuquillo} and T. M. {Jones}},  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},  title={On Microarchitectural Mechanisms for Cache Wearout Reduction},   year={2017},  volume={25},  number={3},  pages={857-871},}
% https://ieeexplore.ieee.org/document/7762198

@INPROCEEDINGS{CF11,  author={C. {Ferri} and D. {Papagiannopoulou} and R. I. {Bahar} and A. {Calimera}},  booktitle={2011 12th Latin American Test Workshop (LATW)},  title={NBTI-aware data allocation strategies for scratchpad memory based embedded systems},   year={2011},  volume={},  number={},  pages={1-6},}
% https://ieeexplore.ieee.org/document/5985932

@INPROCEEDINGS{DP13,  author={D. {Papagiannopoulou} and P. {Prasertsom} and I. {Bahar}},  booktitle={International Symposium on Quality Electronic Design (ISQED)},  title={Flexible data allocation for scratch-pad memories to reduce NBTI effects},   year={2013},  volume={},  number={},  pages={60-67},}
% https://ieeexplore.ieee.org/document/6523591


% Mitigation for SAs

@ARTICLE{DK17,  author={D. {Kraak} and M. {Taouil} and I. {Agbo} and S. {Hamdioui} and P. {Weckx} and S. {Cosemans} and F. {Catthoor}},  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},  title={Impact and Mitigation of Sense Amplifier Aging Degradation Using Realistic Workloads},   year={2017},  volume={25},  number={12},  pages={3464-3472},}
% https://ieeexplore.ieee.org/document/8052501

@INPROCEEDINGS{IA19,  author={I. O. {Agbo} and M. {Taouil} and S. {Hamdioui}},  booktitle={2019 IEEE International Test Conference (ITC)},  title={Reliability Modeling and Mitigation for Embedded Memories},   year={2019},  volume={},  number={},  pages={1-10},}
% https://ieeexplore.ieee.org/document/9000175


% Decoders

@INPROCEEDINGS{sw-based,  author={D. H. P. {Kraak} and C. C. {Gürsoy} and I. O. {Agbo} and M. {Taouil} and M. {Jenihhin} and J. {Raik} and S. {Hamdioui}},  booktitle={2019 IEEE Latin American Test Symposium (LATS)},  title={Software-Based Mitigation for Memory Address Decoder Aging},   year={2019},  volume={},  number={},  pages={1-6},}
% https://ieeexplore.ieee.org/document/8704595

@INPROCEEDINGS{hw-based,  author={D. {Kraak} and I. {Agbo} and M. {Taouil} and S. {Hamdioui} and P. {Weckx} and S. {Cosemans} and F. {Catthoor}},  booktitle={2019 IEEE European Test Symposium (ETS)},  title={Hardware-Based Aging Mitigation Scheme for Memory Address Decoder},   year={2019},  volume={},  number={},  pages={1-6},}
% https://ieeexplore.ieee.org/document/8791536

@Article{MJ16,
author="Jenihhin, Maksim
and Squillero, Giovanni
and Copetti, Thiago Santos
and Tihhomirov, Valentin
and Kostin, Sergei
and Gaudesi, Marco
and Vargas, Fabian
and Raik, Jaan
and Sonza Reorda, Matteo
and Bolzani Poehls, Leticia
and Ubar, Raimund
and Medeiros, Guilherme Cardoso",
title="Identification and Rejuvenation of NBTI-Critical Logic Paths in Nanoscale Circuits",
journal="Journal of Electronic Testing",
year="2016",
month="Jun",
day="01",
volume="32",
number="3",
pages="273--289",
abstract="The Negative Bias Temperature Instability (NBTI) phenomenon is agreed to be one of the main reliability concerns in nanoscale circuits. It increases the threshold voltage of pMOS transistors, thus, slows down signal propagation along logic paths between flip-flops. NBTI may cause intermittent faults and, ultimately, the circuit's permanent functional failures. In this paper, we propose an innovative NBTI mitigation approach by rejuvenating the nanoscale logic along NBTI-critical paths. The method is based on hierarchical identification of NBTI-critical paths and the generation of rejuvenation stimuli using an Evolutionary Algorithm. A new, fast, yet accurate model for computation of NBTI-induced delays at gate-level is developed. This model is based on intensive SPICE simulations of individual gates. The generated rejuvenation stimuli are used to drive those pMOS transistors to the recovery phase, which are the most critical for the NBTI-induced path delay. It is intended to apply the rejuvenation procedure to the circuit, as an execution overhead, periodically. Experimental results performed on a set of designs demonstrate reduction of NBTI-induced delays by up to two times with an execution overhead of 0.1 {\%} or less. The proposed approach is aimed at extending the reliable lifetime of nanoelectronics.",
issn="1573-0727",
doi="10.1007/s10836-016-5589-x",
}

@inproceedings{traber2016pulpino,
  title={PULPino: A small single-core RISC-V SoC},
  author={Traber, Andreas and Zaruba, Florian and Stucki, Sven and Pullini, Antonio and Haugou, Germain and Flamand, Eric and Gurkaynak, Frank K and Benini, Luca},
  booktitle={3rd RISCV Workshop},
  year={2016}
}
@inproceedings{guthaus2001mibench,
  title={MiBench: A free, commercially representative embedded benchmark suite},
  author={Guthaus, Matthew R and Ringenberg, Jeffrey S and Ernst, Dan and Austin, Todd M and Mudge, Trevor and Brown, Richard B},
  booktitle={Proceedings of the fourth annual IEEE international workshop on workload characterization. WWC-4 (Cat. No. 01EX538)},
  pages={3--14},
  year={2001},
  organization={IEEE}
}
@article{rzepa2018comphy,
  title={Comphy—A compact-physics framework for unified modeling of BTI},
  author={Rzepa, Gerhard and Franco, Jacopo and O’Sullivan, Barry and Subirats, Alexandre and Simicic, Marco and Hellings, Geert and Weckx, Pieter and Jech, Markus and Knobloch, Theresia and Waltl, Michael and others},
  journal={Microelectronics Reliability},
  volume={85},
  pages={49--65},
  year={2018},
  publisher={Elsevier}
}

@book{kundert2006designer,
  title={The designer’s guide to spice and Spectre{\textregistered}},
  author={Kundert, Ken},
  year={2006},
  publisher={Springer Science \& Business Media}
}
